Macroeconomic Effects of Active Labour Market Policies: A Novel Instrumental Variables Approach

This study evaluates the macroeconomic effects of active labour market policies (ALMP) in Germany over the period 2005 to 2018. We propose a novel identification strategy to overcome the simultaneity of ALMP and labour market outcomes at the regional level. It exploits the imperfect overlap of local labour markets and local employment agencies that decide on the local implementation of policies. Specifically, we instrument for the use of ALMP in a local labour market with the mix of ALMP implemented outside this market but in local employment agencies that partially overlap with this market. We find no effects of short-term activation measures and further vocational training on aggregate labour market outcomes. In contrast, wage subsidies substantially increase the share of workers in unsubsidised employment while lowering long-term unemployment and welfare dependency. Our results suggest that negative externalities of ALMP partially offset the effects for program participants and that some segments of the labour market benefit more than others.

==> Other/Firststage_alo_rate_alo_tot_l6_all.tex <==
\begin{tabular}{l*{6}{c}}
\hline\hline
            &      F-stat&       p-val&   SW F-stat&    SW p-val&   AP F-stat&    AP p-val\\
\hline
pr\_alo\_tot\_training\_m0\_yd&        7.37&       0.000&       82.83&       0.000&      148.91&       0.000\\
pr\_alo\_tot\_training\_m1\_yd&        7.36&       0.000&       83.05&       0.000&      119.29&       0.000\\
pr\_alo\_tot\_training\_m2\_yd&        7.53&       0.000&       70.10&       0.000&      155.55&       0.000\\
pr\_alo\_tot\_training\_m3\_yd&        7.91&       0.000&       54.22&       0.000&      119.85&       0.000\\
pr\_alo\_tot\_training\_m4\_yd&        8.53&       0.000&       75.19&       0.000&      107.89&       0.000\\
pr\_alo\_tot\_training\_m5\_yd&        8.96&       0.000&       54.76&       0.000&      141.11&       0.000\\
pr\_alo\_tot\_training\_m6\_yd&        8.22&       0.000&       95.28&       0.000&      308.71&       0.000\\
pr\_alo\_tot\_tm\_m0\_yd&        5.86&       0.000&       84.33&       0.000&      466.41&       0.000\\
pr\_alo\_tot\_tm\_m1\_yd&        6.43&       0.000&       58.57&       0.000&      181.07&       0.000\\
pr\_alo\_tot\_tm\_m2\_yd&        6.02&       0.000&       89.97&       0.000&      263.28&       0.000\\
pr\_alo\_tot\_tm\_m3\_yd&        5.90&       0.000&       80.67&       0.000&      212.13&       0.000\\
pr\_alo\_tot\_tm\_m4\_yd&        5.20&       0.000&      100.86&       0.000&      236.60&       0.000\\
pr\_alo\_tot\_tm\_m5\_yd&        6.57&       0.000&       82.74&       0.000&      224.88&       0.000\\
pr\_alo\_tot\_tm\_m6\_yd&        5.50&       0.000&       77.20&       0.000&      318.88&       0.000\\
pr\_alo\_tot\_wagesub\_m0\_yd&       18.11&       0.000&       50.36&       0.000&      501.92&       0.000\\
pr\_alo\_tot\_wagesub\_m1\_yd&       21.15&       0.000&       30.30&       0.000&      142.33&       0.000\\
pr\_alo\_tot\_wagesub\_m2\_yd&       19.43&       0.000&       25.77&       0.000&      169.41&       0.000\\
pr\_alo\_tot\_wagesub\_m3\_yd&       22.96&       0.000&       31.99&       0.000&      202.55&       0.000\\
pr\_alo\_tot\_wagesub\_m4\_yd&       22.50&       0.000&       24.43&       0.000&       83.62&       0.000\\
pr\_alo\_tot\_wagesub\_m5\_yd&       24.06&       0.000&       41.05&       0.000&      160.93&       0.000\\
pr\_alo\_tot\_wagesub\_m6\_yd&       17.29&       0.000&       75.60&       0.000&      541.26&       0.000\\
\hline\hline
\end{tabular}


==> Other/Firststage_alo_rate_alo_tot_l6_main_00_50.tex <==
\begin{tabular}{l*{6}{c}}
\hline\hline
            &      F-stat&       p-val&   SW F-stat&    SW p-val&   AP F-stat&    AP p-val\\
\hline
pr\_alo\_tot\_training\_m0\_yd&        7.98&       0.000&      103.98&       0.000&      123.14&       0.000\\
pr\_alo\_tot\_training\_m1\_yd&        7.85&       0.000&       86.29&       0.000&      114.50&       0.000\\
pr\_alo\_tot\_training\_m2\_yd&        7.82&       0.000&       82.15&       0.000&      126.32&       0.000\\
pr\_alo\_tot\_training\_m3\_yd&        8.37&       0.000&       62.74&       0.000&      112.40&       0.000\\
pr\_alo\_tot\_training\_m4\_yd&        8.04&       0.000&       68.05&       0.000&       98.23&       0.000\\
pr\_alo\_tot\_training\_m5\_yd&        8.95&       0.000&       58.66&       0.000&       98.77&       0.000\\
pr\_alo\_tot\_training\_m6\_yd&        8.32&       0.000&       97.18&       0.000&      284.41&       0.000\\
pr\_alo\_tot\_tm\_m0\_yd&        7.90&       0.000&       98.11&       0.000&      456.56&       0.000\\
pr\_alo\_tot\_tm\_m1\_yd&        8.81&       0.000&       79.91&       0.000&      203.58&       0.000\\
pr\_alo\_tot\_tm\_m2\_yd&        8.10&       0.000&      120.55&       0.000&      335.19&       0.000\\
pr\_alo\_tot\_tm\_m3\_yd&        7.97&       0.000&      115.60&       0.000&      261.70&       0.000\\
pr\_alo\_tot\_tm\_m4\_yd&        7.11&       0.000&      122.15&       0.000&      262.33&       0.000\\
pr\_alo\_tot\_tm\_m5\_yd&        8.71&       0.000&      119.82&       0.000&      275.61&       0.000\\
pr\_alo\_tot\_tm\_m6\_yd&        6.50&       0.000&      147.97&       0.000&      307.52&       0.000\\
pr\_alo\_tot\_wagesub\_m0\_yd&       19.74&       0.000&      119.50&       0.000&      416.70&       0.000\\
pr\_alo\_tot\_wagesub\_m1\_yd&       22.53&       0.000&       82.17&       0.000&      196.22&       0.000\\
pr\_alo\_tot\_wagesub\_m2\_yd&       19.29&       0.000&      115.24&       0.000&      219.52&       0.000\\
pr\_alo\_tot\_wagesub\_m3\_yd&       20.32&       0.000&       74.25&       0.000&      230.60&       0.000\\
pr\_alo\_tot\_wagesub\_m4\_yd&       21.51&       0.000&       83.00&       0.000&      150.84&       0.000\\
pr\_alo\_tot\_wagesub\_m5\_yd&       23.62&       0.000&      105.58&       0.000&      166.55&       0.000\\
pr\_alo\_tot\_wagesub\_m6\_yd&       19.91&       0.000&      126.39&       0.000&      551.49&       0.000\\
\hline\hline
\end{tabular}


==> Other/Firststage_emp_unsub_rate_alo_tot_l6_all.tex <==
\begin{tabular}{l*{6}{c}}
\hline\hline
            &      F-stat&       p-val&   SW F-stat&    SW p-val&   AP F-stat&    AP p-val\\
\hline
pr\_alo\_tot\_training\_m0\_yd&        7.53&       0.000&       93.15&       0.000&      151.98&       0.000\\
pr\_alo\_tot\_training\_m1\_yd&        8.84&       0.000&       86.89&       0.000&      125.11&       0.000\\
pr\_alo\_tot\_training\_m2\_yd&        8.36&       0.000&       68.86&       0.000&      142.71&       0.000\\
pr\_alo\_tot\_training\_m3\_yd&        8.23&       0.000&       56.47&       0.000&      120.68&       0.000\\
pr\_alo\_tot\_training\_m4\_yd&        8.42&       0.000&       72.29&       0.000&      102.74&       0.000\\
pr\_alo\_tot\_training\_m5\_yd&        9.27&       0.000&       55.88&       0.000&      145.68&       0.000\\
pr\_alo\_tot\_training\_m6\_yd&        8.37&       0.000&       99.16&       0.000&      325.43&       0.000\\
pr\_alo\_tot\_tm\_m0\_yd&        5.93&       0.000&       85.23&       0.000&      458.03&       0.000\\
pr\_alo\_tot\_tm\_m1\_yd&        6.48&       0.000&       58.06&       0.000&      179.52&       0.000\\
pr\_alo\_tot\_tm\_m2\_yd&        6.03&       0.000&       84.58&       0.000&      262.99&       0.000\\
pr\_alo\_tot\_tm\_m3\_yd&        5.82&       0.000&       82.62&       0.000&      211.71&       0.000\\
pr\_alo\_tot\_tm\_m4\_yd&        5.21&       0.000&      104.77&       0.000&      233.82&       0.000\\
pr\_alo\_tot\_tm\_m5\_yd&        6.54&       0.000&       83.89&       0.000&      226.75&       0.000\\
pr\_alo\_tot\_tm\_m6\_yd&        5.60&       0.000&       79.29&       0.000&      331.38&       0.000\\
pr\_alo\_tot\_wagesub\_m0\_yd&       17.66&       0.000&       54.91&       0.000&      551.75&       0.000\\
pr\_alo\_tot\_wagesub\_m1\_yd&       18.18&       0.000&       30.00&       0.000&      151.30&       0.000\\
pr\_alo\_tot\_wagesub\_m2\_yd&       17.33&       0.000&       27.23&       0.000&      173.34&       0.000\\
pr\_alo\_tot\_wagesub\_m3\_yd&       21.54&       0.000&       29.53&       0.000&      202.18&       0.000\\
pr\_alo\_tot\_wagesub\_m4\_yd&       22.47&       0.000&       25.55&       0.000&       78.95&       0.000\\
pr\_alo\_tot\_wagesub\_m5\_yd&       24.44&       0.000&       41.37&       0.000&      166.85&       0.000\\
pr\_alo\_tot\_wagesub\_m6\_yd&       17.48&       0.000&       75.11&       0.000&      513.95&       0.000\\
\hline\hline
\end{tabular}


==> Other/Firststage_emp_unsub_rate_alo_tot_l6_main_00_50.tex <==
\begin{tabular}{l*{6}{c}}
\hline\hline
            &      F-stat&       p-val&   SW F-stat&    SW p-val&   AP F-stat&    AP p-val\\
\hline
pr\_alo\_tot\_training\_m0\_yd&        8.03&       0.000&      109.55&       0.000&      128.88&       0.000\\
pr\_alo\_tot\_training\_m1\_yd&        9.26&       0.000&       75.45&       0.000&      136.92&       0.000\\
pr\_alo\_tot\_training\_m2\_yd&        8.51&       0.000&       76.86&       0.000&      112.48&       0.000\\
pr\_alo\_tot\_training\_m3\_yd&        8.53&       0.000&       66.27&       0.000&      114.17&       0.000\\
pr\_alo\_tot\_training\_m4\_yd&        8.04&       0.000&       68.19&       0.000&       95.99&       0.000\\
pr\_alo\_tot\_training\_m5\_yd&        9.32&       0.000&       58.44&       0.000&      100.86&       0.000\\
pr\_alo\_tot\_training\_m6\_yd&        8.45&       0.000&      105.46&       0.000&      282.05&       0.000\\
pr\_alo\_tot\_tm\_m0\_yd&        7.89&       0.000&       99.76&       0.000&      452.40&       0.000\\
pr\_alo\_tot\_tm\_m1\_yd&        8.74&       0.000&       79.09&       0.000&      198.00&       0.000\\
pr\_alo\_tot\_tm\_m2\_yd&        8.11&       0.000&      117.46&       0.000&      334.83&       0.000\\
pr\_alo\_tot\_tm\_m3\_yd&        7.89&       0.000&      119.03&       0.000&      261.32&       0.000\\
pr\_alo\_tot\_tm\_m4\_yd&        7.07&       0.000&      124.96&       0.000&      259.02&       0.000\\
pr\_alo\_tot\_tm\_m5\_yd&        8.64&       0.000&      121.57&       0.000&      272.76&       0.000\\
pr\_alo\_tot\_tm\_m6\_yd&        6.45&       0.000&      145.31&       0.000&      322.35&       0.000\\
pr\_alo\_tot\_wagesub\_m0\_yd&       18.86&       0.000&      119.24&       0.000&      434.94&       0.000\\
pr\_alo\_tot\_wagesub\_m1\_yd&       19.54&       0.000&       77.48&       0.000&      204.72&       0.000\\
pr\_alo\_tot\_wagesub\_m2\_yd&       17.54&       0.000&      128.89&       0.000&      204.95&       0.000\\
pr\_alo\_tot\_wagesub\_m3\_yd&       19.76&       0.000&       74.08&       0.000&      236.39&       0.000\\
pr\_alo\_tot\_wagesub\_m4\_yd&       22.11&       0.000&       79.27&       0.000&      148.87&       0.000\\
pr\_alo\_tot\_wagesub\_m5\_yd&       24.73&       0.000&      102.26&       0.000&      161.86&       0.000\\
pr\_alo\_tot\_wagesub\_m6\_yd&       19.72&       0.000&      116.44&       0.000&      516.18&       0.000\\
\hline\hline
\end{tabular}


==> Other/Sumstats_controls_prog_outcomes.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{longtable}{l*{1}{rr}}
\caption{Summary statistics, CA\_6000\_995}\\
\hline\hline\endfirsthead\hline\endhead\hline\endfoot\endlastfoot
                &\multicolumn{4}{c}{(1)}                \\
                &\multicolumn{4}{c}{}                   \\
                &     mean&       sd&      min&      max\\
\hline
German          &     0.92&     0.14&     0.00&     1.00\\
german\_cens     &     0.00&     0.00&     0.00&     0.00\\
Female          &     0.49&     0.02&     0.44&     0.58\\
20-29 years     &     0.19&     0.02&     0.10&     0.25\\
30-39 years     &     0.22&     0.03&     0.15&     0.31\\
40-49 years     &     0.30&     0.03&     0.20&     0.40\\
50-64 years     &     0.29&     0.05&     0.19&     0.47\\
No schooling degree or schooling degree without Abitur&     0.85&     0.05&     0.67&     0.95\\
Schooling degree with Abitur&     0.15&     0.05&     0.05&     0.33\\
Without Vocational Training&     0.09&     0.04&     0.01&     0.23\\
Vocational Training&     0.83&     0.05&     0.69&     0.94\\
Academic Degree &     0.08&     0.03&     0.02&     0.20\\
Primary sector and manufacturing&     0.26&     0.07&     0.12&     0.45\\
Construction, retail trade and transportation&     0.31&     0.03&     0.22&     0.45\\
Services and communication&     0.12&     0.03&     0.05&     0.22\\
Education, government work, culture and media&     0.31&     0.04&     0.20&     0.44\\
 Female         &     0.44&     0.05&     0.22&     0.65\\
 20-29 years    &     0.23&     0.04&     0.06&     0.39\\
 30-39 years    &     0.19&     0.03&     0.00&     0.31\\
 40-49 years    &     0.21&     0.03&     0.05&     0.35\\
50-64 years     &     0.38&     0.06&     0.17&     0.60\\
 No schooling degree or schooling degree without Abitur&     0.85&     0.06&     0.00&     0.97\\
 Schooling degree with Abitur&     0.15&     0.06&     0.00&     0.38\\
 Without Vocational Training&     0.20&     0.10&     0.00&     0.42\\
 Vocational Training&     0.73&     0.09&     0.52&     0.95\\
 Academic Degree&     0.07&     0.04&     0.00&     0.23\\
voc\_cens        &     0.00&     0.00&     0.00&     0.04\\
Primary sector and manufacturing&     0.23&     0.06&     0.00&     0.52\\
Construction, retail trade and transportation&     0.39&     0.06&     0.17&     0.70\\
Services and communication&     0.15&     0.04&     0.00&     0.31\\
Education, government work, culture and media&     0.23&     0.05&     0.00&     0.43\\
Programs for longterm unemployed&     0.24&     0.25&     0.00&     2.02\\
Programs for the young&     0.05&     0.03&     0.00&     0.24\\
Other programs  &     0.14&     0.11&     0.01&     0.86\\
Resident Labour Force&185504.78&227658.49& 15940.00&1379753.38\\
Further vocational training&     0.13&     0.06&     0.01&     0.51\\
Short training  &     0.11&     0.09&     0.00&     0.76\\
Wage subsidies  &     0.09&     0.06&     0.01&     0.51\\
Further vocational training&     0.13&     0.05&     0.02&     0.35\\
Short training  &     0.11&     0.07&     0.01&     0.50\\
Wage subsidies  &     0.09&     0.06&     0.01&     0.40\\
Unemployment rate (\% of LF)&     0.03&     0.01&     0.01&     0.12\\
Employment rate (\% of LF)&     0.86&     0.07&     0.57&     0.97\\
Share of welfare recipients (\% of total LF)&     0.08&     0.04&     0.00&     0.27\\
Share in precarious work (\% of total LF)&     0.03&     0.02&     0.01&     0.09\\
Inflow rate into employment (\% of LF)&     0.02&     0.00&     0.01&     0.05\\
Unemployment rate female&     0.03&     0.01&     0.01&     0.10\\
Unemployment rate male&     0.03&     0.01&     0.01&     0.13\\
Unemployment rate u30&     0.03&     0.02&     0.01&     0.14\\
Unemployment rate 30-50 years&     0.03&     0.01&     0.01&     0.12\\
Unemployment rate u30&     0.04&     0.02&     0.01&     0.13\\
Unemployment rate low-educated&     0.03&     0.01&     0.00&     0.12\\
Unemployment rate highly-educated&     0.03&     0.01&     0.00&     0.11\\
Unemployment rate low-skilled&     0.05&     0.02&     0.00&     0.17\\
Unemployment rate medium skilled&     0.03&     0.01&     0.01&     0.12\\
Unemployment rate high-skilled&     0.02&     0.01&     0.00&     0.09\\
Employment rate female&     0.87&     0.06&     0.61&     0.97\\
Employment rate male&     0.85&     0.08&     0.49&     0.97\\
Employment rate u30&     0.83&     0.09&     0.46&     0.97\\
Employment rate 30-50 years&     0.86&     0.07&     0.57&     0.97\\
Employment rate u30&     0.83&     0.08&     0.47&     0.96\\
Employment rate low educated&     0.86&     0.07&     0.57&     1.00\\
Employment rate high educated&     0.86&     0.07&     0.49&     1.00\\
Employment rate low-skilled&     0.74&     0.12&     0.25&     1.00\\
Employment rate medium skilled&     0.87&     0.07&     0.56&     0.98\\
Employment rate high-skilled&     0.88&     0.07&     0.52&     1.00\\
\hline
Observations    &     5980&         &         &         \\
\hline\hline
\end{longtable}
}


==> Other/Table_DL_effects_main_alo_rate_l6.tex <==
            &      effect&          se&       p-val&      effect&          se&       p-val\\
Training\_st &      -0.016&       0.002&       0.000&       0.006&       0.014&       0.686\\
Training\_lt &      -0.010&       0.004&       0.004&      -0.016&       0.012&       0.191\\
SM\_st       &      -0.006&       0.001&       0.000&       0.000&       0.008&       0.985\\
SM\_lt       &      -0.005&       0.002&       0.003&      -0.008&       0.008&       0.340\\
Wagesub\_st  &      -0.032&       0.004&       0.000&      -0.040&       0.012&       0.001\\
Wagesub\_lt  &      -0.023&       0.004&       0.000&      -0.017&       0.009&       0.057\\


==> Other/Table_DL_effects_main_emp_unsub_rate_l6.tex <==
            &      effect&          se&       p-val&      effect&          se&       p-val\\
Training\_st &       0.019&       0.008&       0.017&       0.037&       0.068&       0.589\\
Training\_lt &       0.036&       0.015&       0.020&       0.010&       0.040&       0.814\\
SM\_st       &      -0.003&       0.005&       0.540&      -0.011&       0.026&       0.658\\
SM\_lt       &       0.006&       0.006&       0.327&      -0.000&       0.022&       0.984\\
Wagesub\_st  &       0.013&       0.012&       0.288&       0.018&       0.078&       0.816\\
Wagesub\_lt  &       0.087&       0.014&       0.000&       0.203&       0.034&       0.000\\


==> Other/Table_effects_main_inflow_rate_emp_l6.tex <==
            &      effect&          se&       p-val&      effect&          se&       p-val\\
Lagged\_depvar&       0.065&       0.021&       0.002&       0.059&       0.040&       0.139\\
Training\_st &       0.001&       0.002&       0.748&      -0.015&       0.027&       0.569\\
Training\_lt &       0.003&       0.002&       0.164&      -0.006&       0.008&       0.480\\
SM\_st       &       0.002&       0.001&       0.086&      -0.009&       0.017&       0.605\\
SM\_lt       &       0.002&       0.002&       0.194&      -0.001&       0.006&       0.922\\
Wagesub\_st  &       0.001&       0.002&       0.695&       0.018&       0.018&       0.307\\
Wagesub\_lt  &       0.003&       0.002&       0.059&       0.007&       0.007&       0.279\\


==> Other/Table_effects_rob_main_00_50_l6.tex <==
            &      effect&          se&       p-val&      effect&          se&       p-val\\
Multiplier  &       0.629&       0.038&       0.000&       0.685&       0.013&       0.000\\
Training\_st &       0.000&       0.014&       0.990&      -0.009&       0.029&       0.754\\
Training\_lt &      -0.030&       0.018&       0.086&      -0.022&       0.086&       0.801\\
SM\_st       &       0.002&       0.008&       0.777&      -0.008&       0.021&       0.706\\
SM\_lt       &      -0.004&       0.012&       0.741&       0.003&       0.040&       0.939\\
Wagesub\_st  &      -0.030&       0.010&       0.003&       0.039&       0.054&       0.468\\
Wagesub\_lt  &       0.007&       0.013&       0.557&       0.285&       0.058&       0.000\\

